Improving mid-infrared thermal background subtraction with Principal Component Analysis

Ground-based large-aperture telescopes, interferometers, and future Extremely Large Telescopes equipped with adaptive-optics systems provide angular resolution and high-contrast performance that are superior to space-based telescopes at thermal-infrared wavelengths. Their sensitivity, however, is critically limited by the high thermal background inherent to ground-based observations in this wavelength regime. We aim to improve the subtraction quality of the thermal-infrared background from ground-based observations, using Principal Component Analysis (PCA). We use data obtained with the Nulling-Optimized Mid-Infrared Camera on the Large Binocular Telescope Interferometer as a proxy for general high-sensitivity, AO-assisted ground-based data. We apply both a classical background subtraction -- using the mean of dedicated background observations -- and a new background subtraction based on a PCA of the background observations. We compare the performances of these two methods in both high-contrast imaging and aperture photometry. Compared to the classical background subtraction approach, PCA background subtraction delivers up to two times better contrasts down to the diffraction limit of the LBT's primary aperture (i.e., 350 mas in N band), that is, in the case of high-contrast imaging. Improvement factor between two and three are obtained over the mean background retrieval within the diffraction limit in the case of aperture photometry. PCA background subtraction significantly improves the sensitivity of ground-based thermal-infrared imaging observations. When applied to LBTI's nulling interferometry data, we expect the method to improve the sensitivity by a similar factor 2-3. This study paves the way to maximising the potential of future infrared ground-based instruments and facilities, such as the future 30m-class telescopes.

==> Sections/appli_imaging.tex <==
\section{Application to high-contrast imaging}\label{sec:app_highcontima}

In this section, we present the additional steps and the exact configuration of PCA background subtraction (pre-subtraction, numbers of PCs for background and PSF subtraction) used for HCI processing. Here, the mask size is always set to 9 pixels in radius. Therefore, unlike aperture photometry we did not probe different mask sizes. Another important difference between the aperture photometry analysis and HCI analysis resides in five additional steps described in the following subsections: recentering, filtering, averaging, enlargement and best-curve selection. 

\subsection{Recentering}

As for the mask position, we first determine the star center group per group. Once this first guess value is determined, for more precision in the recentering process, we still allow the algorithm to search for the star center in individual frames around the first guess value. As LBTI provides high stability for the star position, we were able to limit the search for the "real" star center position within a box of 5 pixels around the first guess value (nine times the tip-tilt jitter RMS delivered by the AO system). The recentering in itself is performed with the VIP function for cube recentering with a 2d Gaussian. 

\subsection{Filtering}

In order to obtain the best contrast curves, we remove the bad frames from the dataset, and the corresponding parallactic angle values from the angle vector. In our case, the bad frames are those containing the largest amount of starlight since this is indicative of a large null leak (analog to poor starlight suppression by a coronagraph). To reject those bad frames, we can thus set a maximum threshold in terms of percentage of the star photometry and reject all the frames for which the star photometry is above this threshold. To find the optimal filtering, we tried different percentage of the star photometry (maximum photometry obtained in a 9-pixel aperture) for the threshold. The chosen filtering levels were : 100, 80, 60, 40 and 20$\%$. 

\subsection{Averaging and enlargement}

After the recombination, the datacube is already usable for processing. However, in order to save computational time, we average the frames. We tested averaging groups of frames with group sizes ranging from 10 to 100 and finally selected 100 as we did not observe any significant differences with the non-averaged datacube. Above this number, the number of remaining frames is too low and the contrast curves and final images start to degrade. This is thus in great part tied to the number of frames contained in the $\beta$ Leo dataset. When working with larger datasets, one might still be able to average more frames at once. The data cubes from the two $\beta$ Leo pointings used for image processing thus contained after this averaging step 80 frames and 88 frames, respectively.

The field of view of our datacubes being very narrow compared to the PSF size, we had to enlarge the images artificially to match VIP requirements. VIP requires the ratio of the half of the frame size (61.5 pixels in our case) and the fwhm (18 pixels) of the PSF to be above 4, while the native ratio in our data is 3.4. This condition is set to avoid overlapping injected companions in the image. In order to avoid having to make significant changes to this algorithm, we thus enlarged the images from a size of 123x123 pixels to 200x200 pixels. The artificial part was filled with a random gaussian distribution with the mean and standard deviation computed from the actual data in each individual image. Thus, all artificially enlarged parts are different from one image to another. 

\subsection{Best-curve selection}

For image processing, in order to compare the mean and PCA background subtraction, with as little bias as possible, we used three different processing methods: Without Subtraction of the PSF (WS), Angular Differential Imaging (ADI) and Reference-star Differential Imaging (RDI). The PSF subtraction is performed on the merged datacube for $\beta$ Leo, thus containing the two pointings of the night and thus 168 frames. The averaging step mentioned earlier is performed before we merge the two pointing in order to avoid averaging frames with a large observing time and parallactic angle separation. For this analysis we built one mean background subtracted dataset and thirty PCA background subtracted dataset, with each a different PC number, ranging from 1 to 30.

For the first method (WS), we de-rotate the frames according to their parallactic angles and compute the median image. The contrast curve is directly computed on this final image. For the ADI PSF subtraction, we used the corresponding VIP algorithm with full-frame PCA, in its ADI mode, this time providing the parallactic angle vector for de-rotation. To check for convergence of the PCA, we derived contrast curves for the first N PCs with N ranging from 1 to 10, resulting in ten contrast curves per datacube. For RDI PSF subtraction, we also made use of the same full-frame PCA algorithm, but in its RDI mode. We tried two different calibrators: HD104979 and HD108381. Since this last one was providing significantly better results, we will only display the contrast curves obtained with this calibrator. As for ADI, we computed the contrast curves for principal components ranging from 1 to 10, and thus obtained 10 contrast curves per datacube. 


For mean background subtraction, we obtained 30 contrast curves per filtering with the different libraries of background frames (Sect 2.5.1) and principal components for PSF subtraction. For PCA, we used 30 different principal components for background subtraction, with three different options for pre-subtraction (including none), three different background libraries and 10 different principal components for PSF subtraction, thus obtaining 2700 curves per filtering. In order to easily compare mean and background subtraction, with as little bias as possible, we thus selected each time the best contrast curve among all those obtained for both methods, with and without filtering. 

We first selected the best curves among those obtained for a particular datacube but different principal component number for PSF subtraction. For PCA, among those best curves we selected the optimal principal component for background subtraction (we determine the convergence to happen at 20 PCs), then the best pre-subtraction option (including none). Finally, we selected the best library for both mean and PCA background subtraction. All those best curves selections are automatically done by comparing the sum of all the points along the contrast curves for each configuration.

Finally, we selected the best filtering level in each case and compared them with the best non-filtered contrast curve. In the following section we show only the best results.

==> Sections/appli_photo.tex <==
\section{Application to aperture photometry}\label{sec:app_apertphoto}

 We perform aperture photometry on every frame individually and then perform statistical analysis on the results by group and on the whole data set. For this analysis, we use an empty dataset, with only background. We chose this approach because the ideal residual background is expected to be zero, and we can thus easily compute the deviation from the ideal value. However, in order to remain representative in the methodology used for the background subtraction, we processed this dataset as if a source was present in the data. On the model of the $\beta$ Leo dataset, we recreated groups of a thousand frames which we then consider to be source exposures or background exposures. The choice of which groups is considered source or background exposures has been made arbitrarily. However, as in a dataset containing a star, we alternate between a group of source exposures and a group of background exposures. In addition, as we would have for a scientific target dataset, we used a mask during PCA background subtraction, and a background annulus for mean background subtraction. These results are presented and discussed in Sect. 5.1. In our case the mask, the background annulus and the photometric aperture are centered on the frame center, however in the case of a real dataset containing a source, since we are not recentering the images for aperture photometry, those three elements should be centered on the source center.

To minimize over-subtraction of the astrophysical source in the data during PCA, we mask the region of interest.  Since the source can be extended, we explore a range of circular photometric aperture sizes and matching mask sizes. Similarly, for aperture photometry after the mean background subtraction, the background annulus must be chosen carefully according to the size of the photometric aperture and the size of the astrophysical source. In the following, we distinguish two cases described in the following subsections : the general case and the case specific to exozodiacal dust observations.

\subsection{General}

In this case, we adapt the mask size to the source extension. We explore a range of source sizes from a point source (FWHM in our data 17.98 pixels) to 32 pixels in radius.  For the point-source case we use a photometric aperture of 8 pixels in radius (\citealt{defrere_nulling_2016}, \citealt{ertel_hosts_2018,ertel_hosts_2020}) and a mask for PCA of 9 pixels in radius.  For larger photometric apertures, we set the mask size to that of the photometric aperture.  For the classical background subtraction, we set the inner radius of the background annulus to one pixel larger than the radius of the photometric aperture and the outer radius so that the area of the background annulus matches that of the photometric aperture.  This is done to obtain the background measurements from pixels as close as possible to the photometric region.  It produces the most optimistic performance, while depending on the exact use case wider or larger background annuli may be necessary.

\subsection{Exozodiacal dust}

One of the main motivations of this study is to evaluate the performance of PCA background subtraction in the context of exozodiacal dust measurements from the HOSTS survey.To explore this use case, we add to our analysis a modified approach that resembles that used by \cite{ertel_hosts_2020}. A range of photometric apertures was used (\citealt{ertel_hosts_2020}, \citealt{defrere_hosts_2021}).  Among those apertures, three stand out in particular:  8-pixel, 13-pixel, and conservative.  The 8-pixel aperture is the smallest reasonable aperture assuming unresolved emission.  The 13-pixel aperture is optimized for maximum S/N assuming a dust distribution analog to the Solar system as most of the emission is then concentrated close to the star and at most marginally resolved by the single-telescope aperture.  The conservative aperture includes most of the conceivable dust emission and is adjusted to each individual star (luminosity and distance).  The additional aperture sizes are used to constrain the radial distribution of the marginally resolved dust emission in case of a detection.  The PCA mask and background annulus used after mean background subtraction need to be adjusted according to the conservative aperture, irrespective of the actual photometric aperture used, in order to avoid subtracting extended dust emission.  If the conservative aperture is used, the general case described above and the exozodi case are identical.

==> Sections/methodo.tex <==
\section{Mean vs PCA background subtraction}\label{sec:methodo}

We present here a succinct overview of the two background-subtraction methods investigated in this article for both aperture photometry and high-contrast imaging: the mean background subtraction and the PCA background subtraction.

In the case of the mean background subtraction approach, we compute the mean of a sequence of dedicated background exposures and then subtract it from every on-source exposure. The high-contrast analysis, to search for circumstellar emission, is then performed without further treatment of the background. 
The aperture photometry analysis is performed using a background annulus to estimate the background under the photometric aperture. The photometry in this annulus is then subtracted from the photometry in the region of interest. The resulting photometry is then used for further analysis. This approach is extensively described in \textbf{ \citet{defrere_2016}.}

The PCA approach is a statistical method which allows one to reconstruct the data as a basis of eigenvectors corresponding to the level of variance in the data. It thus determines the dominant features of this set of data. The number of principal components used in this analysis determines the strength of the features that the analysis will consider, from the most dominant to the less significant ones. Thus, it determines the level of detail the analysis will be able to reconstruct. This method is commonly used for high-contrast imaging to remove the stellar Point Spread Function (PSF, \citealt{amara2012}, \citealt{2012ApJ...755L..28S}, \citealt{amara2015}). Here, we use it to better estimate and remove the sky background, similar to the approach used by \cite{hunziker_pca-based_2018}. We first proceed to a pre-subtraction analogous to the mean background subtraction (see Section \ref{sec:pre_subtraction}). We then perform PCA on background exposures. This determines the eigenvectors (or principal components), onto which the science images are projected. In order to avoid source over-subtraction, a mask on the star is introduced during this step (see Section \ref{sec:masking_star}). With this technique, an optimal correction is computed for, and subtracted from, each on-source science image. This technique allows for an additional background removal to the classical subtraction for high-contrast analysis. In the case of aperture photometry, it replaces the background annulus used in the mean background subtraction. PCA is indeed capable of reconstructing the background at the position of  the star, which constitutes a more sophisticated estimate than the background annulus. 
